Towards Building Economic Models of Conversational Search

Various conceptual and descriptive models of conversational search have been proposed in the literature -- while useful, they do not provide insights into how interaction between the agent and user would change in response to the costs and benefits of the different interactions. In this paper, we develop two economic models of conversational search based on patterns previously observed during conversational search sessions, which we refer to as: Feedback First where the agent asks clarifying questions then presents results, and Feedback After where the agent presents results, and then asks follow up questions. Our models show that the amount of feedback given/requested depends on its efficiency at improving the initial or subsequent query and the relative cost of providing said feedback. This theoretical framework for conversational search provides a number of insights that can be used to guide and inform the development of conversational search agents. However, empirical work is needed to estimate the parameters in order to make predictions specific to a given conversational search setting.

==> Previous_models.tex <==
\vspace{-2mm}
\subsection{An Economic Model of Conversational Search - Feedback After}
Given Model 2 (Feedback After), we can extended the original economic model of search by adding in feedback ($F_{2}$), such that a user issues a query, assess $A_{2}$ items, then provides feedback to refine the query, followed by assessing another $A$ items. The process of giving feedback and assessing, then repeats this $F_{2}$ times. For this kind of conversational interaction,  we can define the gain to be proportional to the number of queries and the number of rounds of feedback per query and the number of assessments per query or round of feedback:
\begin{equation}
    \label{eq:gain_model1}
    g_{2}(Q_{2}, F_{2}, A_{2}) =  Q_{2}^\alpha. (1+F_{2})^{\gamma_{2}}. A_{2}^\beta 
\end{equation}
As before, $\alpha$ and $\beta$ denote the efficiency of querying and assessing, while $\gamma_{2}$ expresses the efficiency of providing feedback. We can see that if $F=0$ (e.g. no feedback), then the model reverts back to the original model in Eq.~\ref{eq:original}. 
\begin{equation}
    \label{eq:cost_model1}
    c_{2}(Q_2, F_{2}, A_2) = Q_{2}.C_q + Q_{2}.F_{2}.C_f + Q_{2}.(1+F_{2}).A_{2}.C_a
\end{equation}

The cost function is also extended to include the rounds of feedback, and the additional assessments per feedback round, where if $F_{2}=0$ then the cost model reverts back to the original cost model. The amount of feedback per query will depend on the cost of the feedback, and it's relative efficiency ($\gamma_{2}$).
So if $\gamma_{2}=0$ and $F_2>0$ then there is no additional benefit for providing feedback -- only added cost.

To determine the optimal number of assessments and feedback, for a given level of gain $G$ where we want to minimise the total cost to the user given $G$ we create the following objective function:

\begin{equation}
    \label{eq:delta_1}
    \Delta_{2} = Q_{2}.C_q + Q_{2}.F_{2}.C_f + Q_{2}.(1+F_{2}).A_{2}.C_a -\lambda( Q_{2}^\alpha. (1+F_{2})^\gamma_{2}. A_{2}^\beta - G)
\end{equation}

By finding the partial derivatives and solving the equations we obtain the following expressions for the optimal number of assessments ($A^{\star}$), and the optimal number of rounds of feedback ($F_{2}^{\star}$):

\begin{equation}
A_{2}^{\star} = \frac{\beta.C_q + \beta.F_{2}.C_f }{(\alpha-\beta).(F_{2}+1)C_a}
\end{equation}

\begin{equation}
F_{2}^{\star} = \frac{\beta.C_q + (\alpha-\beta).A_{2}.C_a }{(\alpha-\beta).A_{2}.C_a + \beta.C_f}\label{eq_f2}
\end{equation}

Given these expressions, we can see that there is a relationship between providing feedback and assessing. And, if we set $F_{2}=0$, then the model, again, falls back to the original model in Eq.~\ref{eq:original}.

Inspecting the equations, we can further see that the optimal number of assessments (per query or per round of feedback) is dependent on the number of rounds of feedback.  Specifically, assuming feedback is to be given/requested (i.e. $F_{2}>0$), then if the cost of performing the feedback increases, on average, a user should examine more items per query and per round of feedback. If the cost of assessing items increases, then, on average, a user should examine fewer items per query/feedback. Intuitively, this makes sense, as it suggests a user should invest more in refining their need to bring back a richer set of results, than inspecting additional results for the current query or round of feedback.
Now, if the relative efficiency of assessing increases, then a user should examine more items per query or per round of feedback, \todo{while if the relative efficiency of giving feedback increases, then a user should examine fewer items per query/feedback}.  

In terms of the feedback, we can see that the number of rounds of feedback is dependent upon the cost of querying -- this is because querying is the natural alternative to providing another round of feedback. Here, we can see that as the cost of querying increases, then, on average, users should provide more feedback. While if the cost of giving feedback increases, then, on average, users should provide less feedback. If the relative efficiency of giving feedback increases, then users should provide more feedback, while if the relative efficiency of querying increases then users should provide less feedback (i.e. queries are more efficient). For Model 2, as the efficiency of assessing $\beta$ improves and tend to $\alpha$, then $F_{2}$ will be become negative -- suggesting no feedback. On the other hand, for Model 1, as $\beta$ improves and tends to $\alpha$, the amount of feedback $F_1$ that can be given will increase. 







==> out.tex <==
Model 1 - Feedback After. This conversational search pattern is based on presenting results to the user, and then asking for feedback to further refine or expand the query. For example, The user asks about Almond Milk (query), and the agent responses, by first providing an overview of almond milk (assessment), before presenting follow up / feedback questions (i.e. would you like to know about the benefits, alternatives, recipes, etc.). The user and agent engage in a number of round of feedback and assessments, until the user issues a new query.

Model 2 - Feedback First. This conversational search pattern is once a user provides a query, the agent asks a series of clarifying questions (feedback) before presenting results (assessments). For example, the user asks about almond milk, and the agent asks if the user wants to know about is benefits, alternatives, etc. before then presenting the answers.


\subsection{An Economic Model of Search}
In the economic model for search proposed in ~\cite{azzopardi2011}, the gain the user receives is proportional to the number of queries that they issue (Q) and the number of items that they assess (A) per query. The exponents $\alpha$ and $\beta$ denote the relative efficiency of querying and assessing. If $\alpha=\beta=1$ then for every item inspected the user would get a gain of one. However, in practice, $\alpha$ and $\beta$ are less than one, and so the more querying or more assessing naturally leads to diminishing returns. i.e. assessing one more item is less likely to yield as much gain as the previous item, and similarly for issuing another query as the next result less may contain previously seen items, previously seen information, or simply the user has found most of the relevant items (e.g. each relevant item found, means there is one less in the pool for that topic).


\begin{equation}
    g(Q, A) = Q^\alpha. A^\beta     \label{eq:original}
\end{equation}
    \begin{equation}
    c(Q, A) = Q.C_q + Q.A.C_a
\end{equation}
For the cost to the user, it is also proportional to the number of queries issued and the total number of items inspect (i.e. $Q \times A$), where the cost per query is $C_q$ and the cost per assessment is $C_a$. By framing the problem as an optimisation problem, where the user wants a certain amount of gain, then the number of assessments per query that would minimize the overall cost to the user is:
\begin{equation}
A^{\star} = \frac{\beta.C_q}{(\alpha-\beta).C_a}
\end{equation}
Here, we can see that as the cost of querying increases, then, on average, users should go deeper. While if the cost of assessing increases, on average, users should assess fewer items per query. If the relative efficiency of querying (alpha) increases, then users should assess fewer items per query, while if the relative efficiency of assessing (beta) increases then the users should assess more. Moreover, there is a natural trade-off between querying and assessing, such that to obtain a given level of gain $g(Q,A)=G$ then as the $A$ increases, $Q$ decreases, and vice versa.


In order to develop an economic model of conversational search, we need to make a series of assumptions about the affordances of the system, and how a user can interact with the system. First, we assume that our conversational system only reacts to user's requests (similar to most conversational systems that are already available on the market). Therefore, the system only produces responses given the user's input. The system can respond in one of two ways: (i) request additional feedback to clarify or specify the user's query, or (ii) report answers back to the user given their query. A user, therefore, will either (ii) issue a new query, (ii) provide feedback on a query, or (iii) receive answers. We shall further assume that the conversation takes place over a limited-bandwidth channel (e.g., voice-only), and so the costs and benefits of the interactions are particularly salient.  From the user's point of view they want to maximise the amount of gain that they receive, for a given cost, while the system want to ensure that this user's experience is optimised. So for this reason, it may be that the user decides not to give further feedback given a request by the system, or decides not to listen to subsequent results in the list -- or -- alternatively, the system may decide not to request any further feedback, nor provide any more results. However, on average, we are interested in finding out and understanding, what would be the optimal course of interaction? More specifically, how many queries should the user pose, how many requests for feedback should the system ask (or user respond to), and how many answers should the system provide (or the user listen to)? 

It is worth noting that the described system and its usage is only one possible conversational system -- and it provides a limited set of interactions. However it provides a basis for exploring the aforementioned questions, and is based on the empirical derived model \textbf{QRFA} model proposed in~\cite{vakulenko2019qrfa}. It also enables us to explore the different trade-off between querying, answering, and clarifying, as hypothesised in~\cite{azzopardi2018conceptual}. 
